Adversarial Neural Trip Recommendation

Trip recommender system, which targets at recommending a trip consisting of several ordered Points of Interest (POIs), has long been treated as an important application for many location-based services. Currently, most prior arts generate trips following pre-defined objectives based on constraint programming, which may fail to reflect the complex latent patterns hidden in the human mobility data. And most of these methods are usually difficult to respond in real time when the number of POIs is large. To that end, we propose an Adversarial Neural Trip Recommendation (ANT) framework to tackle the above challenges. First of all, we devise a novel attention-based encoder-decoder trip generator that can learn the correlations among POIs and generate well-designed trips under given constraints. Another novelty of ANT relies on an adversarial learning strategy integrating with reinforcement learning to guide the trip generator to produce high-quality trips. For this purpose, we introduce a discriminator, which distinguishes the generated trips from real-life trips taken by users, to provide reward signals to optimize the generator. Moreover, we devise a novel pre-train schema based on learning from demonstration, which speeds up the convergence to achieve a sufficient-and-efficient training process. Extensive experiments on four real-world datasets validate the effectiveness and efficiency of our proposed ANT framework, which demonstrates that ANT could remarkably outperform the state-of-the-art baselines with short response time.

==> 4_copy.tex <==
% Since we have real trajectories from user, we can regard the real trajectories as ground truth to train our model.
Now given a trip query, the time-aware trip generator is able to plan a trip for the user.
However, the generated trip may fail to achieve the maximum objective defined in Equation \ref{obj}.
Obviously, the real trip from the user can be considered to achieve the maximum objective.
In other words, the more similar a generated plan is to a real trajectory, the larger objective it will achieve.
So a discriminator that is capable to distinguish the real trip with the planned trip is essential.

In the training process, the trip generator first produces a trip and then the discriminator makes a distinction between the planned trip with the real trip and scores the generated plan.
A higher score means that the user is more likely to follow the generated plan.
That is to say, the trip generator $G_\theta$ aims to achieve a high score from the discriminator $D_\phi$, where $\theta$ and $\phi$ are the parameters of generator and discriminator respectively.

\subsubsection{Discriminator}
As our goal is to maximize the probability that the user will follow the planned trip.
We can directly estimate the probability with the discriminator $D_\phi$.
The discriminator takes the real trip and the trips generated by the trip generator and outputs the scores, which could be used to guide the optimization of the trip generator.
Compared to the complicated task for the trip generator, the task for the discriminator is a much easier binary classification task.
Following \cite{goodfellow2014generative}, we train the discriminator $G_\theta$ and the generator $D_\phi$ alternately for enhancing both discriminator and generator.

% To balance the training process for generator and discriminator, we're supposed to design a discriminator that is not so powerful with low computational cost.
% In other words, if the discriminator is too powerful, the reward signal it generates is too low for the plan generator to learn efficiently.
% So we apply a simple one-layer Gated Recurrent Unit (GRU) \cite{cho2014learning} followed by a two-layer feed-forward network as the discriminatory to capture the sequential information from the input and distinguish them.

% \subsubsection{Embedding}. Same as the embedding in plan generator, given the user u and a real trajectory or a plan $\{l_1, l_2, \ldots, l_n \}$, we use a simple linear transform to integrate the user and the POIs $l_i$ with its category $c_i$ for embedding:
We denote all trajectories as $P_{data}$. As a binary classification task, 
\hide{we computes loss for the discriminator as:
\begin{align}
    \mathcal{L}_D = - \sum  \limits_{(S, I) \in P_{data}} & [\ \log D_\phi(S| I; \theta) \notag \\ & + 
    \log (1 - D_\phi(S| I; \theta)]
\end{align}}
\li{
we train the discriminator $D_\phi$ as follows:
\begin{align}
    \mathop{\mathrm{min}}\limits_{\phi} - \mathbb{E}_{S\sim P_{data}}[\log D_\phi(S)] - \mathbb{E}_{S\sim G_\theta}[\log (1 - D_\phi(S))]
\end{align}
}

\subsection{Training}
Though the proposed framework is composed of a generator and a discriminator, following the GAN structure, the standard training algorithm is not capable to our framework. 
Compared to standard GAN structure, the discrete output from the generator, which is sampling based on the probability distribution makes the loss from discriminator non-differentiable and can't optimize the generator by back-propagation.

\subsubsection{Reinforcement Learning based Training}
Thus, we consider the plan generation procedure as a sequential decision making process and update the planning generator by using reinforcement learning techniques.
From the perspective of reinforcement learning, the POIs that are selected  $S_{0:t}$ until time step $t$ and the context embedding can be regarded as \emph{state} and the output probability can be seen as a stochastic \emph{policy}.
So the score from the discriminator can be seen as a reward signal, which can be used to optimize the generator
and we train our generator with \emph{policy gradient} \cite{sutton2018reinforcement}.

A benefit of using discriminator as reward signal is that we can dynamically update the discriminator to further optimize the generator.
After our plan generator produces enough plans, we will update the discriminator to distinguish real trajectories from generated plans better.
Once we get a new discriminator, we will train the plan generator with new reward signal from the new discriminator. Given a instance $S$, Section \ref{generator} defines a probability distribution $p_{\theta} (S | S)$, where we can sample to make a plan $S$.
In order to train the plan generator, we define the loss
$
    \mathcal{L}(S) =  \mathbb{E}_{p_{\theta}(S | S)}
    [D_\phi(S | S)]
$.
Follow the REINFORCE algorithm, we generate the policy gradient as:
\begin{equation}
    \nabla \mathcal{L}(I) = \nabla \mathbb{E}_{p_{\theta}(S | I)} [D_\phi(S | I)] = 
     \nabla \mathbb{E}_{p_{\theta}(S | I)} [D_\phi(S | I) \nabla \log p_\theta(S|I)]
\end{equation}
On the basis of gradient above, we can update the parameters $\theta$ of our plan generator by gradient ascent with proper learning rate.

\subsubsection{Pre-training}
However, learning directly from such a sparse reward is sample inefficient and hard to converge.
Following \cite{yu2017seqgan}, we utilize the real trajectories to pre-train our generator to make the best use of data.

We can learn the policy from the real trajectory, which is named \emph{learning from demonstration} in reinforcement learning \cite{silver2010learning}.
\emph{Learning from demonstration} is helpful to solve the sample-inefficiency and speed up the training process by utilizing the demonstrations.
% However, learning only from demonstrations can lead to a sub-optimal policy when the demonstrations are sub-optimal.
% So after learning from demonstrations, we gain a baseline policy.
% On the basis of the baseline policy, we can learn a better policy directly to maximize the reward signal with policy gradient.

Actually, learning from demonstration is a method belonging to supervised learning, which uses the interaction records from an experienced expert as the ground truth \cite{silver2010learning}.
In our problem we use the real trajectory from the user as ground truth and maximize the probability of the real trajectory by using maximum likelihood estimation (MLE).

% We denote all the instances as  $P_{data}$ and for each instance we represent it as a two-tuple $(S, I)$, where $S$ represents the real trajectory and $I$ represents the corresponding user, starting POI, time budget, POI candidate set.

For each trajectory $Y \in P_{data}$ and corresponding problem instance $S$, the probability of outputting the trajectory $Y$ from the plan generator is:
\begin{equation}
    P(Y \mid S) = \prod \limits_{t=1}^{|Y|} P(Y_t \mid Y_{1:t-1}, S; \theta)
\end{equation}
Then we define the loss by MLE:
\begin{equation}
    \mathcal{L}_S = - \sum \limits_{Y \in P_{data} } \sum \limits_{t=1}^{|Y|} P(Y_i \mid Y_{1:t-1}, S; \theta)
\end{equation}

During inference, the decoder needs the previous POI to select the next POI while we have no access to the true previous POI.
To prevent the gap between training and inference, we select POI by sampling with the probability distribution during training.
So the loss we compute during training is:
\begin{equation}
    \mathcal{L}_S = - \sum \limits_{Y \in P_{data}} \sum \limits_{t=1}^{|Y|} P(Y_t | S_{0:t-1}, S; \theta)
\end{equation}
where  $S_{0:t-1}$ is the actual generated plan in the training process.

To sum up, we first pre-train our plan generator by leveraging demonstration data. To further improve the plan generator, we use reward signal from the discriminator to directly optimize our generator.
The discriminator is also updated during the process, which provides a better guidance for improving the generator.
